RAF: Holistic Compilation for Deep Learning Model Training

As deep learning is pervasive in modern applications, many deep learning frameworks are presented for deep learning practitioners to develop and train DNN models rapidly. Meanwhile, as training large deep learning models becomes a trend in recent years, the training throughput and memory footprint are getting crucial. Accordingly, optimizing training workloads with compiler optimizations is inevitable and getting more and more attentions. However, existing deep learning compilers (DLCs) mainly target inference and do not incorporate holistic optimizations, such as automatic differentiation and automatic mixed precision, in training workloads. In this paper, we present RAF, a deep learning compiler for training. Unlike existing DLCs, RAF accepts a forward model and in-house generates a training graph. Accordingly, RAF is able to systematically consolidate graph optimizations for performance, memory and distributed training. In addition, to catch up to the state-of-the-art performance with hand-crafted kernel libraries as well as tensor compilers, RAF proposes an operator dialect mechanism to seamlessly integrate all possible kernel implementations. We demonstrate that by in-house training graph generation and operator dialect mechanism, we are able to perform holistic optimizations and achieve either better training throughput or larger batch size against PyTorch (eager and torchscript mode), XLA, and DeepSpeed for popular transformer models on GPUs.

==> Figures/fig-compile.tex <==
\begin{figure*}[!tb]
	\centering
	\includegraphics[width=\linewidth]{./Figures/src/raf-compile.pdf}
	\caption{\system Compilation Flow \protect\zhen{If we do not plan to claim distributed training, Auto Data Parallel should not be here}}
	\label{fig:compile}
\end{figure*}

==> Figures/fig-ir.tex <==
\begin{figure}[tbh]
    \centering
    \begin{lstlisting}
let %t1 = conv2d(%x, %w);
let %t2 = add(%t1, %b);
let %t3 = relu(%t2);
%t3
    \end{lstlisting}
    \caption{A graph of Conv2D+Bias+ReLU defined in A-Normal Form.}
    \label{fig:anf}
\end{figure}

\begin{figure}[tbh]
    \centering
    \begin{lstlisting}
%1 = conv2d(%x, %w);
%2 = add(%1, %b);
relu(%2);
    \end{lstlisting}
    \caption{A graph of Conv2D+Bias+ReLU defined in Graph Normal Form.}
    \label{fig:gnf}
\end{figure}


==> Figures/fig-jit.tex <==
\begin{figure}[tbh]
	\centering
	\includegraphics[width=\linewidth]{./Figures/src/jit.pdf}
	\caption{Just-In-Time Compilation in Runtime \protect\haichen{move to runtime?}}
	\label{fig:jit}
\end{figure}

==> Figures/fig-runtime.tex <==
\begin{figure}[tbh]
	\centering
	\includegraphics[width=\linewidth]{./Figures/src/raf-runtime.pdf}
	\caption{VM Runtime}
	\label{fig:runtime}
\end{figure}


==> Sections/old.3.design.tex <==
\section{Design Principles}\cody{deprecated and merged to Intro}
\label{sec:design}
%\yida{maybe rename it to design principles? 1) user friendly; 2) flexible graph-level optimization; 3) fully explore efficient backend; 4) exhaust optimization opportunities. The current setting is to some degree duplicated with what we describe in Sec. 4.}

Considering the challenges presented in the previous section, this section discusses the design principles for deep learning compilers to training workloads.
%\yida{can we map the philosophies to challenges? Some philosophy is for non training specific challenges (e.g., op dialect), so we should think of a way.}

\noindent\textbf{\#1. Holistic optimizations.}
As illustrated in \textit{Challenge~1}, training graphs include more computations in addition to the forward inference. Instead of limiting the optimization scope to the training graphs generated by deep learning frameworks, optimization scope of DLCs should be extended to training graph construction, including automatic differentiation, automatic mixed precision, and distribution.

%\yida{let's emphasize we only need a vanilla model, so it saves a lot of user work. For example, users don't need to write in a DeepSpeed format. Can we compare the line of model code?}
%\cody{per discussion. there's no difference from user's point of view.}
%As illustrated in \autoref{sec:bg_dlc}, we argue that getting control of the entire procedure of generating and executing training graph of the model is the key to full optimization
%\yida{do we really argue that in that subsection?}.
%Therefore, unlike existing works, \system should jointly consider the auto differentiation, training graph optimization, code generation, and compiled module execution.
%In other words, \system will take the original forward model along with the user semantic (i.e., training/inference, data type, memory budget, etc.\yida{do we demonstrate these settings later?}) to perform self-contained transformations.

\noindent\textbf{\#2. Flexible graph-level optimization.} 
\cody{not sure how to claim this point...}
Existing deep learning frameworks choose different graph-level IRs to facilitate their own usage.
For example, PyTorch~\cite{paszke2019pytorch} and TVM~\cite{chen2018tvm} use dataflow IR for easy traversal and manipulation.
Dataflow IR is suitable for graph-level optimization passes such as operator fusion, expression simplification, and dead code elimination.
For another example, XLA~\cite{xla} uses A-normal form (ANF) IR which can represent the execution order of each node.
Compared to dataflow IR, ANF is better at certain passes such as auto-differentiation, CUDA multi-stream scheduling, memory planning, and tensor rematerialization.
In order to better support more optimization passes, \system is designed to use both IRs, each of which is used exclusively at a stage.

\noindent\textbf{\#3. Support both kernel libraries and tensor compilation.} 
Since most state-of-the-art DLCs focus on inference, their tensor-level optimization and code generation are optimized for inference workloads, which are forward operators with a single batch size.
However, modern DLCs may fail to generate competitive kernels over hand-crafted ones on 1) backward operators and 2) operators with large batch size.
Since it may take a while for DLCs to involve its tensor-level optimization match kernel library performance, it is more practical to let the compiler backend dispatch an operator to either kernel libraries or tensor compilation depending on their so far best result quality.


%A kernel library or a code generator is as a {\em backend} in \system.
% We notice that there are usually multiple ways to implement the tensor computation of the model training even for the same platform, e.g., cuBLAS/cuDNN, CUTLASS, and TVM-generated CUDA code for the same platform such as NVIDIA GPU, and the number of implementations keeps growing.
% The best performance is usually achieved by the combined usage of multiple implementations.
% In addition, we observe that more and more accelerators emerge, each of which has its own backend.
% Therefore, \system is designed to be extensible to multiple backends, and more importantly, flexible to invoke different backends for the same workload in a hybrid mode.
% The complexity in the backend dispatching comes from the fact that none of backends can achieve the best performance across all cases.
% For instance, the GEMM kernel in CUTLASS performs better than that in cuBLAS library for float16 data type, while being shy of cuBLAS at float32.
% Furthermore, every new training accelerator (e.g., AWS Trainium, Google TPU) has at least one specific codegen.
% As a result, \system should enable the flexible incorporation of different backends as needed.

% \noindent\textbf{\#4. IR and backend coupling.} \yida{can we name this philosophy ``holistic optimization''?}\cody{merged to #1}
% Ideally, IR should be backend-independent, but some optimizations have to be performed with the backend considerations.
% For example, CUTLASS and TVM backend both support operator fusion, but their fusion patterns are different from each other.
% If we apply the operator fusion optimization pass without considering backends, it is likely that the optimized graph can be only applicable to one backend, leading to sub-optimal performance.
% Another case is that in the mixed precision training, one backend can have its customized mixed precision operators while others don't support. 
% As a result, we need to couple backends and IR optimization together for best performance.

\yida{any design philosophy for distributed training?}

==> Sections/old.implementation.tex <==
\section{Design and Implementation}
\label{sec:impl}

In this section, we illustrate \system implementations and discuss how the design philosophy presented in the previous section is integrated.

\subsection{System Overview}
\label{sec:impl_overview}

\input{Figures/fig-compile}

\autoref{fig:compile} presents an overview of the \system compilation flow.
As mentioned in the previous section, \system accepts a vanilla forward (i.e., inference) model to fully control the training specific behaviors.
Specifically, \system traces the forward model to 1) build an intermediate representation (IR), and 2) extract model parameters.
Then it performs auto-differentiation to generate the back propagation logic, and applies user-specified training configurations, such as the type of optimizer (e.g., SGD, Adam, etc), whether to enable automatic mixed precision (AMP), whether to enable data parallelism, and so on.

We highlight that unlike other frameworks that separate forward inference, back propagation, and parameter updating to different modules, \system maintains a single all-in-one IR module to perform an entire training iteration for a mini-batch together.
In other words, the inputs of the IR module include a mini-batch in training data sets, learnable parameters, and optimizer states.
After executing the IR module, the learnable parameters and optimizer states are in-place updated.
The benefit of putting it all together is to let the underlying IR transformation passes have a global view to perform analysis and optimization.

With the all-in-one IR module, \system applies a series of IR transformation passes for optimizations, organized in two sequences in BBNF and ANF representations, respectively.
We apply the first sequence of the IR to optimize the dataflow, transform the IR to ANF, and apply the second sequence to optimize the operator execution order and memory footprint.
The details of IR with different forms are introduced in \autoref{sec:impl_ir}.
Afterwards, the optimized IR module will then be compiled to \system VM bytecode for execution.

\input{Figures/fig-runtime}

\autoref{fig:runtime} depicts the VM execution flow in a training loop.
Before kicking off the training loop, \system initializes a VM instance such as loading bytecode, initializing registers and memory pool.
Then it enters the training loop.
For each training iteration, the VM interprets the bytecode to manipulate registers, manage memory pool, and invoke the corresponding kernels.
In particular, when an operator or a closure (i.e., a fused operator) is visited for the first time, VM leverages just-in-time (JIT) compilation to generate and cache the executable binary.
To support extensible backends, \system introduces the concept of operator dialects that associate each base operator (e.g., \texttt{Matmul}) to backend-specific dialect operators (e.g., \texttt{cblas.matmul}, \texttt{cublas.matmul}, \texttt{cutlass.matmul}, or \texttt{tvm.matmul}).
A base operator can be dispatched to a dialect operator in compile phase by an optimization pass, or in runtime phase by the VM, providing high flexibility for developers to make the best decision. The details are illustrated in \autoref{sec:impl_dialect}.
We note that both VM initialization and JIT compilation are one-time overheads, so it will not hurt the user experience as training a model usually needs thousands to millions iterations.

\subsection{Frontend}
\label{sec:impl_frontend}

We observe that users tend to use interactive interface provided by PyTorch~\cite{paszke2019pytorch} to write and tune the deep learning models for training. 
As a compilation-based framework, however, \system's native frontend deviates drastically from the imperative programming paradigm PyTorch has. 
In our setting, the compilation and execution of models are separated explicitly, which makes it difficult for users to print intermediate results or make modification to their models. 
What's worse, in this way, users are required to interact with RAF in a way that is different from what they are used to in PyTorch, and it takes huge amount of work to run their existing models or training scripts with \system.

To alleviate the issue, \system incorporates Lazy Tensor Core (LTC) ~\cite{suhan2021lazytensor} as its imperative frontend.
%, referred to as RAZOR (RAf via laZy tenOR). 
With this frontend, users can easily convert their PyTorch training scripts to \system with only 2-3 lines of code. 
One of the required modifications is to specify a \system device, via which PyTorch tensors and operations on the device would be staged and executed lazily. 
The other is that users should explicitly synchronize at the end of each training loop, which flushes the staged operators and forces the weight updates. 
The APIs provided by our frontend is entirely modelled after LTC, so users can take full advantage of the flexible imperative user interface highlighted by PyTorch. 
For example, they can print intermediate tensors for debugging purposes, clip their gradients, and apply various optimizers such sgd~\cite{bottou2010large} and Adam~\cite{kingma2014adam}.

Following LTC, we adopt the tracing technique to convert an imperative model into a \system one. 
Each operator is staged as a symbol in \system IR and the evaluation of it is lazy: the symbol is not evaluated until its result is needed. 
For example, its evaluation will be triggered if users print it out or invoke the synchronization API explicitly. 
\system's frontend is designed as an out-of-tree extension to PyTorch and can be easily incorporated with officially released PyTorch packages without changing upstream PyTorch codebase. 
%It hooks the operators on the specified \system device to customized tracing APIs and does not need any modification to the upstream PyTorch codebase. 
We did not directly reuse the LTC in PyTorch as it was original designed for XLA which traces models into the HLO IR.
However, \system adopts an IR setting which allows us to perform holistic optimization that HLO IR does not do.
%Although this frontend is essentially equivalent to LTC, we failed to fully reuse its code because it is originally designed for XLA and it traces models into HLO IR, which is the IR used by XLA. We extend LTC and represent models with RAF IR, which allows us to perform holistic optimization.

\subsection{IR}
\label{sec:impl_ir}

The intermediate representation (IR) design in \system follows the design principles in Relay~\cite{roesch2019relay} and adopts the strongly-typed functional IR. 
It consists of a few core functional expressions, including local/global var, call, let, function, tuple, and if-else, and a set of operators to represent different computation in the neural networks.
Although some existing frameworks such as PyTorch embraces runtime model interpretation without strictly type checking to preserve the flexibility, we argue that a strong type system is still necessary to enable advanced optimizations. For example, almost all \texttt{*\_like} operators (e.g., \texttt{zeros\_like} and \texttt{reshape\_like}) can be simplified if the type of the reference tensor is static, so that the memory footprint can be significantly reduced.

\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.5\linewidth}
\centering
\begin{lstlisting}
let %t1 = conv2d(%x, %w);
let %t2 = add(%t1, %b);
let %t3 = relu(%t2);
%t3
\end{lstlisting}
\vspace{-1em}
\caption{\label{fig:anf}}
\end{subfigure}
\begin{subfigure}[b]{0.35\linewidth}
\begin{lstlisting}
%1 = conv2d(%x, %w);
%2 = add(%1, %b);
relu(%2);
\end{lstlisting}
\vspace{-3pt}
\caption{\label{fig:gnf}}
\end{subfigure}
\caption{A graph of conv2d + bias + relu defined in both (a) A-Normal Form (ANF) and (b) Graph Normal Form (GNF).}
\label{fig:anf-gnf}
\end{figure}

As depicted in \autoref{fig:compile}, \system performs optimization on two IR forms: {\em A-Normal Form} (ANF) and {\em Graph-Normal Form} (GNF). 
Expressions in the ANF IR are bound to a variable using \texttt{let} (\autoref{fig:anf}), while in GNF IR, the program is formatted in the dataflow graph fashion, and expressions are embedded as arguments in the subsequent expressions (\autoref{fig:gnf}).
Usually a compiler only contains one IR form. For example, the IR in the MLIR follows three-address SSA representation, and Node IR in PyTorch JIT compiler uses GNF. 

The reason that \system has two different IR forms is because each form has its advantage and disadvantage with regard to optimization passes. 
ANF IR form binds each expression to a variable and implies the order of expressions through the sequence of \texttt{let} statements. 
Therefore, it is easy to encode extra information in the IR associated with variables, i.e., tape information in the AutoDiff pass (\autoref{sec:impl_autodiff}), and friendly to optimizations that requires the information of execution order, such as memory planning (\autoref{sec:impl_memory}). 
However, the enforcement of expression order also makes it harder for optimization that needs to re-order the expressions such as operator fusion (\autoref{sec:impl_fusion}). 
And that's where GNF IR form wins over ANF. 
GNF IR form represents a dataflow graph and optimization passes on top of GNF IR can easily traverse the graph and make modifications. 

\system enables comprehensive optimization passes as well as reduces their development effort by having two IR forms, but it also brings a new challenge when transforming between ANF and GNF.
The transformation from ANF to GNF could potentially lose information of the execution order and attributes associated to let-bound variables.
On the other hand, when converting from GNF to ANF, the ordering of expressions makes impact to the performance and operator parallelism (see more details at \autoref{sec:impl_graph_sch}).
To address this challenge, \system carefully places the optimization passes in different stages and makes sure that the transition between ANF and GNF doesn't lose any information by encoding it in the IR and recovering the information in the later stage.

%Extend Relay

%GNF - pros/cons

%ANF - pros/cons

%Challenges when transforming from GNF to ANF and vice versa.

\subsection{Operator dialects}
\label{sec:impl_dialect}

With the availability of various implementations on the same platform, the kernel selection process becomes inevitably complicated and hard to achieve optimal performance. What's making it worse is that more and more backend implementation now introduce the capability of operator fusion such as cuDNN v8 \cite{xxx} and CUTLASS \cite{yyy} while supporting different fusion patterns.

Motivated by MLIR~\cite{lattner2021mlir}, we introduce the operator dialects to address this issue. Similar to the dialect language in MLIR, we register each backend implementation as a new dialect in the IR, e.g., ``cudnn'',  ``tvm'', etc.,  and enable the customization for operators in each dialect. But different from MLIR which views all backends as dialects, \system comes with a set of pre-defined operators as base operators. This can reduce the effort in the addition of a new dialect operator by sharing certain operator attributes from base operators such as type relation function and users do not need to write the code for translation between 
every dialect pair as MLIR requires. Nonetheless, it still provides the flexibility that allows dialect operators to have customized semantics via attribute tables, as described below, and more importantly, enables different fusion patterns for each dialect (detailed in \autoref{sec:impl_fusion}).

% Revisit the challenge of supporting/dispatching ops to different backends (performance/memory/fusion considerations), and present op dialect mechanism.

% Why do we need operator dialects? \\
% A: to handle different backends and different fusion

% Use TVM as the comprehensive support.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/src/dialect_op.pdf}
    \caption{A dialect operator associated with one dialect is registered to a base operator with a dispatching priority. A dialect is only enabled on certain devices.}
    \label{fig:dialect-op}
\end{figure}

As depicted in \autoref{fig:dialect-op}, a dialect operator is registered to a base operator with a dispatching priority. The priority is used in the optimization pass and at runtime to determine which backend implementation is used to achieve best performance\yida{may need to elaborate}. The priority value can be pre-defined by developers based on prior experiences or derived from profiling results. A dialect operator is also associated with a dialect. For example, \texttt{tvm.conv2d} that belongs to dialect \texttt{tvm} is registered to the base operator \texttt{conv2d} with priority 10. In addition, a dialect is allowed be only enabled on certain devices. For instance, \texttt{tvm} can be used on both CPU and GPU, while \texttt{cudnn} and \texttt{cutlass} is only available for CUDA. If a dialect isn't available for the compilation target, all dialect operators in this dialect won't be used in the IR or dispatched to at runtime.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/src/dialect_op_attr.pdf}
    \caption{The attribute table for base and dialect operators. Dialect operators can have attributes inherited from base operators, attributes overwritten on top of base operators, and customized attributes that are specific to dialect operators.}
    \label{fig:dialect-op-attr}
\end{figure}

Every operator including both base and dialect operators has its own attribute table. The attribute table of a base operator contains common attributes that could potentially share across its dialect operators, such as argument schema, type relation functions, etc., as shown in \autoref{fig:dialect-op-attr}. Most of attributes of dialect operators can inherit from base operators so that it significantly reduces the developer effort to add new dialect operators (blue items in \autoref{fig:dialect-op-attr}). On the other hand, dialect operators can overwrite certain attribute value on top of the base operators and have its own specific attributes (red and green items respectively). For example, in \autoref{fig:dialect-op-attr}, \texttt{cudnn.dropout} has a different type relation function as the cuDNN implementation needs to reserve extra space for the states.

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{./Figures/src/jit.pdf}
	\caption{Just-In-Time Compilation in Runtime \protect\haichen{move to runtime?}}
	\label{fig:jit}
\end{figure}

\subsection{AutoDiff}
\label{sec:impl_autodiff}
\yida{We didn't mention why autodiff should be done in the compiler, instead of relying on the framework.}
Auto differentiation (AutoDiff) pass applies the chain 
rule to the given forward (inference) graph to generate the backward graph for training.
In the AutoDiff pass, we evaluate the chain rule from outputs to inputs (i.e., the reverse mode AutoDiff). This is because 
for deep learning, in which large tensors of input parameters are typically updated using 
gradient descent on a scalar output, the number of inputs is significantly larger than the number of outputs.
The reverse mode’s time complexity scales with the number of output.

We employ source code transformation with a closure-based method~\cite{pearlmutter2008reverse} to perform the differentiation. 
The transformation proceeds as follows: each operator in forward graph is transformed by an adjoint function, which computes the derivative
with respect to the inputs given the derivatives with respect to the outputs. In order to ensure that the transformation 
can be applied again on the transformed graph (for the computation of second-order derivatives), it must be able to handle functions
with free variables. So each adjoint function returns the partial derivatives with respect to
the inputs of the original function, as well as an ordered set of partial derivatives with respect to the
free variables.

For each operator used in the forward graph, an adjoint function is registered. Developers have the freedom to choose the following two approaches to implement the adjoint function at different granularity:

\noindent\textbf{A subgraph:} We could use other operators directly to composite the adjoint function. These operators will be separate nodes in the IR, and we can let optimization passes such as operator fusion determine the optimization strategy. For example, they might be fully fused to be a single fused operator, partially fused to be a few fused operators, or even partially fused with other operators.

\noindent\textbf{A single operator:} If the gradient calculation of an operator has to be manually optimized to achieve better performance and memory consumption, then developing a new backward operator explicitly is better. For example, the backward of widely used operators such as \texttt{Conv2D} have been heavily optimized in cuDNN for GPU. In this case, we simply register new operators \texttt{Conv2D\_dx} and \texttt{Conv2D\_dw} and associate them to the cuDNN implementations.

%\zhen{We should mention that we register operators for different backends and assign different priorities in somewhere (should be in op dialect part, and then mention it again here). For instance, the conv2d\_dx has both cuDNN backend and TVM backend. On Nvida GPU, cuDNN backend has higher priority.}
%\cody{I was thinking about that too but didn't mention in because I can't make it clear enough, and it seems not that critical in this subsection.}
%\yida{How about mentioning this in the op dialect subsection?} \zhen{Yep, I also think it should be mentioned in op dialect part}.
% Developers could also use the domain specific language (DSL) to specify the arithmetic expression of gradient calculation, or even leverage the auto-gradient feature in TVM to automatically figure out the gradient equation. With this approach, we will obtain a single operator in the IR, and it is 

The AutoDiff pass will generate closure(s) and append the closure(s) to forward graph, the return of the whole graph is the forward output and closure(s). 
After AutoDiff pass, The the Inline Backward pass will be executed, which will perform the lifting and inline the backward graph to the forward graph.  
\cody{this seems too detail even for the technical report?}

\subsection{Graph-level optimization}
\todo{Mention that we also have VM in addition to the interpreter, so we can perform graph-level optimization instead of graph interpretation.}

\todo{Then present some important passes. Candidates: AutoDiff, FuseOps, MemoryPlan, AutoCast, Rematerialization, GradInputSelect/InplaceUpdate (and more?)}

\subsubsection{Graph Scheduling}
\label{sec:impl_graph_sch}

\zhen{what is this subsection for?}\cody{this is for ANF scheduling, such as multi-stream scheduling. But we may not need this section so let's just leave it here for now.}

\input{Sections/4.opt_fusion}

%This design simplify the implementation of both fusion and AudoDiff pass: the AutoDiff pass does not need to 

\subsubsection{Inplace Updating}
Inplace updating can save reduce memory consumption and eliminate the unnecessary memory allocations, 
which introduce allocation overhead and may cause fragmented memory. We implement an inplace update pass
to achieve that purpose.  
Even though the variables in IR
are immutable, we can mark \texttt{may\_share} in the variable for operators that have inplace update 
character, so that inputs and outputs may share the memory and perform inplace update.
For instance, once the binary operator \texttt{add} has inplace argument set to be true, the 
inplace update pass marks the output tensor to share the memory with the first input tensor.
Then during runtime, VM will reuse the first input and save the output to it instead of allocating a 
new tensor for \texttt{add}.
The inplace update pass also benefits training operators with side effect.
For example, batch norm keeps track of global states, i.e., running variance and running mean. 
During training, we reuse input memory to update the running variance and running mean by 
indicating the batch norm operator as an inplace update operator. 

\subsubsection{Memory Optimization}
\label{sec:impl_memory}
One of the most important challenge for deep learning training model systems is to deal with the memory footprint.
Different from the intermediate tensors in inference graphs that usually have a short liveness and can be released immediately, most intermediate tensors generated in the forward phase of training graphs have to be used in the backward phase, making their liveness long.
Consequently, it is easy for training graphs to run out of device memory during the forward phase.
To reduce the memory footprint, \system incorporates several memory optimization techniques inspired by existing works.
We introduce them along with \system specific consideration as follows. 

\noindent{\textbf{Gradient Memory Optimization: }}
As mentioned in \autoref{sec:impl_autodiff}, every forward operator has a corresponding adjoint function registered to calculate the gradient of the operator.
In general, an adjoint function of a forward operator $y = f(x)$ is $g = f'(x, y, dy)$, where $x$ is the forward input tensor, $y$ is the forward output tensor, $dy$ is the gradient of the next forward operator, and $g$ is the gradient of the current operator.

\yida{is it similar to the last paragraph of \autoref{sec:impl_fusion}}On the other hand, according to arithmetic characteristic, we can calculate the gradient of certain operators with only $x$ or $y$ tensor but not both.
Taking $y = tanh(x)$ as an example, its gradient can be calculated by $g = dy\times(1-tanh(x)-tanh(x)) = dy\times(1-y-y)$.
Accordingly, we could simplify the adjoint function to $g = tanh\_dx(y, dy)$, and release the input tensor $x$ in the forward phase.
These operators are firstly named \textit{invertible operators} by DeepSpeed \cite{}.
In \system, \cody{I wish to say something like we can automatically realize unnecessary tensors and DeepSpeed is manually checked, but we also manually check now...}

\noindent{\textbf{Memory planning and gradient rematerialization: }}
Releasing unused tensors immediately after their last use is critical for deep learning model training systems to maintain the memory footprint.
Existing frameworks with eager semantics such as PyTorch~\cite{paszke2019pytorch} leverage either garbage collection or reference counting.
With a compiler solution in \system, we are capable of analyzing an entire graph and leveraging the accurate tensor liveness to free them.

In the case that no immediate tensors can be released but still cannot fit into the device memory, gradient rematerialization, also called gradient checkpointing in PyTorch, is adopted as a solution to trade memory with performance.
Unlike PyTorch that relies on model developers to determine the checkpoints and replays every operators between two checkpoints, \system again leverages liveness analysis to perform static memory tracing to only rematerialize necessary tensors, which minimizes the performance overheads when enlarging the maximum supported batch size.

\subsection{Runtime}

\system adopts virtual machine-based approach to build its runtime, similar to~\cite{shen2021nimble, tfrt}.
There are 3 major benefits from using virtual machine: 1) it's lightweight with negligible overhead; 2) it's flexible enough to encode all sorts of optimization in the runtime; and 3) it's versatile and portable to different platforms including cloud and edge devices.
\system improves the virtual machine design in Nimble~\cite{shen2021nimble} by having more advanced features, including the support of CUDA stream \cite{cuda_stream} and CUDA graph \cite{cuda_graph}, and the integration of a profiler.
\system also simplifies the dynamic type inference at runtime by directly re-using the type relation functions registered to the operator attributes (\autoref{sec:impl_dialect}) and getting rid of extra runtime type functions required in Nimble.

To support CUDA stream, \system introduces 4 new CUDA stream and event-related instructions: \texttt{CudaSetStream}, \texttt{CudaAddEvent}, \texttt{CudaWaitEvent}, and \texttt{CudaStreamBarrier}. At runtime, \system also maintains a stream pool and event pool to switch between CUDA streams and wait for events. This enables the operator parallelism and improves the performance for models that has branches such as Inception~\cite{szegedy2016rethinking} and NasNet~\cite{zoph2018learning}.
CUDA graph provides a graph definition mechanism that merges multiple GPU kernel launches into one and thus reduces the kernel launch overhead.
\system integrates the virtual machine with the CUDA graph that captures a CUDA graph in the first run and invokes the graph instead of interpreting VM instructions in the subsequent runs.

\begin{figure}
\centering
\begin{subfigure}{\linewidth}
\includegraphics[width=\linewidth]{Figures/src/prof_lvl1.png}
\caption{Level 1}
\label{fig:prof-lv1}
\end{subfigure}
\begin{subfigure}{\linewidth}
\includegraphics[width=\linewidth]{Figures/src/prof_lvl2.png}
\caption{Level 2}
\label{fig:prof-lv2}
\end{subfigure}
\caption{Profile trace visualization}
\label{fig:vm_profile}
\end{figure}

The virtual machine in \system supports different levels of profiling.
At the default profiling level (level 1), it records the latency of kernel execution on both CPU and GPUs and certain meta data of kernels such as kernel names, input shapes, and execution stream (only applicable to GPU).
While in profiling level 2, the profiler also records the latency in the instruction interpretation so that developers can further debug the overhead brought by the VM.
\autoref{fig:vm_profile} shows the visualization of the profile logs using profiling level 1 and 2.
\system also provides analysis tools to analyze the profile results for performance debugging.

%Why Nimble. Profiler, visualizer.


==> Sections/old.opt_fusion.tex <==

\subsubsection{Fusion}
\label{sec:impl_fusion}
Operator fusion combines multiple operators into a single kernel and can greatly reduce kernel execution time by avoiding the data transfer of intermediate results between cache and main memory.
It is particularly effective for GPUs and specialized accelerators.
As we mentioned before, multiple backends have the capabilities for operator fusion and their fusion patterns are different from each other.
For example, CUTLASS could fuse matrix multiplication (GEMM) kernel with bias add and element wise activation, while TVM code generation has a much broader fusion patterns as long as they fit into its fusion rules.
However, though TVM can fuse more operators together, the performance of TVM generated kernels could be inferior to CUTLASS generated ones.
Therefore, we need to address the trade-off between more operator fusion and better kernel performance, and choose among multiple fusion patterns that can be applied to different subgraphs.

To accommodate different levels of fusion capabilities for all backends, \system divides the operator fusion optimization into two categories: {\em pattern-based fusion} and {\em rule-based fusion}. 
For example, fusion for CUTLASS and cuDNN backends belong to pattern-based category as they only support limited fusion patterns. 
On the other hand, TVM belongs to rule-based fusion as it performs general-purpose operator fusion based on rules \cite{chen2018tvm}.

For pattern-based fusion, \system provides an interface for developers to register fusion patterns. 
Thanks to operator dialect described in \autoref{sec:impl_dialect}, we can attribute each pattern to a specific dialect, to indicate which backend is used for code generation of the fused operators. 
Each pattern is associated with a priority, which determines the order of application of these fusion patterns.
We also set priorities to rule-based fusion like TVM and the operator fusion pass applies these fusion patterns and fusion rules one at a time based on their priorities in a descending order.
The orders of pattern matching will lead to different fused graphs and can have different performance.
Currently, the priorities are set by developers based on heuristics, but in the future, we plan to derive the priorities from profiling results and perform search on all possible graph partition solutions based on the fusion patterns and fusion rules to find optimal fusion plans.

\begin{table}[t]
\centering
\begin{tabular}{c|c|c}
    \toprule
    Pattern / Rules & Dialect & Priority \\ \midrule
    conv2d + bias + relu (fp16) & cutlass & 15 \\
    conv2d + bias + relu & cudnn (>=8) & 12 \\
    conv2d & cudnn & 10 \\
    conv2d + bias + relu & cutlass & 8 \\
    TVM fusion rules & tvm & 5 \\
    \bottomrule
\end{tabular}
\caption{Fusion patterns and rules with priorities \label{tab:fusion-pattern}}
\end{table}

\begin{figure}[t]
\centering
\begin{subfigure}{\linewidth}
\begin{lstlisting}
%1 = mnm.op.conv2d(%x: f16, %w: f16);
%2 = mnm.op.relu(%1);
%3 = mnm.op.add(%2, %y);
%4 = mnm.op.multiply(%3, %z);
\end{lstlisting}
\vspace{-6pt}
\caption{Pre-fused program}
\label{fig:unfused}
\end{subfigure}

\begin{subfigure}{\linewidth}
\begin{lstlisting}
%1 = fn(%p0, %p1, dialect="cutlass") {
  %2 = mnm.op.cutlass.conv2d(%p0, %p1);
  %3 = mnm.op.cutlass.relu(%2)
};
%4 = %1(%x: f16, %w: f16);
%5 = mnm.op.add(%4, %y);
%6 = mnm.op.multiply(%5, %z);
\end{lstlisting}
\vspace{-6pt}
\caption{After applied CUTLASS fusion pattern}
\label{fig:fuse-cutlass}
\end{subfigure}

\begin{subfigure}{\linewidth}
\begin{lstlisting}
%1 = fn(%p0, %p1, dialect="cutlass") {
  %2 = mnm.op.cutlass.conv2d(%p0, %p1);
  %3 = mnm.op.cutlass.relu(%2)
};
%4 = %1(%x: f16, %w: f16);
%5 = fn(%p0, %p1, %p2, dialect="tvm", primitive=1) {
  %6 = mnm.op.tvm.add(%p0, %p1);
  %7 = mnm.op.tvm.multiply(%6, %p2)
};
%8 = %5(%4, %y, %z);
\end{lstlisting}
\vspace{-6pt}
\caption{After applied TVM fusion rules}
\label{fig:fuse-tvm}
\end{subfigure}

\caption{Operator fusion example}
\label{fig:fusion-example}
\end{figure}

We use a simple example (\autoref{fig:unfused}) to show how operator fusion takes action and applies the fusion patterns and rules.
\autoref{tab:fusion-pattern} gives an example of a few fusion patterns related to \texttt{conv2d} and TVM fusion rules with priorities.
First, the CUTLASS fusion pattern for fp16 data type in the fusion table has the highest priority.
The optimization pass finds a matching in the program and then replaces the matched sub-graph by a fused operator with dialect \texttt{"cutlass"} and a function call, shown in \autoref{fig:fuse-cutlass}.
After that, no patterns other than TVM fusion rules can be found applicable to the transformed program.
\autoref{fig:fuse-tvm} shows the final program after the fusion optimization.

% Operator fusion combines multiple operators into a single kernel without saving the 
% intermediate results in memory. This optimization can greatly reduce kernel execution time, 
% particularly in GPUs and specialized accelerators.
% \zhen{Do we need to say something about CUTLASS fusion support? Not sure where is the best place to mention that}
% \haichen{Yes, we need to have the CUTLASS fusion here. I'll add and probably rewrite part of the fusion subsection after I finish the op dialect part.}
% For TVM backends, we implement a rule based fusion pass to fuse adjacent operators. Two operators
% meeting two requirements can be fused together: (1) The intermediate data will not be used
% in the future. (2) the two operators fall in certain categories and follow our predefined rules.
% Specifically, we identify six
% categories of operators: 1) Element-wise (e.g., \texttt{ReLu}), which applies an function of each element of the tensor.
% 2) broadcast operator (e.g., broadcast add: add a tensor and a scalar), 
% which can always map output axis to the input in order to a single input axis.
% 3) injective (e.g., add two same size tensors), it is one-to-one map, which can always 
% injectively map output axis to a single input axis. 
% 4) reduction (e.g., \texttt{sum}), which combines values from many items in a tensor.
% 5) complexout-fusable (e.g., \texttt{Conv2D}), which can fuse element-wise map to output, 
% and (6) opaque (e.g., sort), which cannot be fused with any operator.

% The generic rules to fuse operators are as follows.
% Multiple injective operators can be fused into another injective operator. 
% A reduction operator can be fused with input injective operators (e.g., fuse scale and sum). 
% Operators such as \texttt{Conv2D} are complex-out-fusable, and we can fuse element-wise operators, 
% e.g., \texttt{ReLu}, to its output. 
% Element-wise operator can be fused with all operators except for the opaque.
% We apply these rules to fuse the adjacent operators.

Performing fusion for training graph is more challenging than inference. Some intermediate data
is not needed to be stored for the inference, but is needed in backward to calculate the gradients, 
In order to get the data dependency for the whole training graph, we apply fusion pass after AutoDiff pass. 
If the intermediate data appears in the backward graph, the corresponding operator that generates the data will not be fused with
the following operators\yida{this assumes no recomputation.}. 

There are some more room to further increase the fusion opportunities. When we register
the adjoint functions, the adjoint function takes both primal operator's input and output as parameters by default. 
Actually, this is not always the case. For some special operators, only input or output is enough to calculate the gradient.
For instance, for $z=ReLu(y)$, we can use either $y$ or $z$ to calculate the gradient instead of both $z$ and $y$.
We use a GradInputSelect pass to set the input arguments for each adjoint function. 
For $y = Conv2D(x,w); z = ReLu(y)$ case, we use the GradInputSelect to set $Conv2D\_dx$ taking inputs (i.e., $x$ and $w$) 
and $ReLu\_dx$ using output, i.e., $z$, so that intermediate data $y$ is not needed in the backward graph and $Conv2D$ and $ReLu$
can be fused.

==> Tables/tbl-pass-list.tex <==
\begin{table}
 \label{tab:pass}
 \caption{Passes and their IR format}
    \centering
    \begin{tabular}{|l|l|}
    \hline
        Pass Name & IR Format \\ \hline
        LiftBranchBody & ANF \\ \hline
        FlattenClosure & ANF \\ \hline
        Autodiff & ANF \\ \hline
        InlineBackward & ANF \\ \hline
         &  \\ \hline
        ToGraphNormalForm & Any → GNF \\ \hline
        ToBasicBlockNormalForm & GNF → BBNF \\ \hline
         &  \\ \hline
        AutoDataParallel & BBNF \\ \hline
        DeadCodeElimination & BBNF \\ \hline
        FuseOps & BBNF \\ \hline
        GradInputSelect & BBNF \\ \hline
        AutoCast & BBNF \\ \hline
        FoldConstant & BBNF \\ \hline
        PartitionGraph & BBNF \\ \hline
        AnnotateTarget & BBNF \\ \hline
        MergeCompilerRegions & BBNF \\ \hline
        CanonicalizeOps & BBNF \\ \hline
         &  \\ \hline
        ToANormalForm & Any → ANF \\ \hline
        ManifestAlloc & ANF \\ \hline
        InplaceUpdate & ANF \\ \hline
        DeviceAnalysis & ANF \\ \hline
        Lower to VM & ANF \\ \hline
         &  \\ \hline
        InferType & Any \\ \hline
        Substitute & Any \\ \hline
        SimplifyExpr & Any \\ \hline
    \end{tabular}
\end{table}

